Critical Thinking: Which Kinds of Complexity Govern Optimal Reasoning Length?

Large language models (LLMs) often benefit from verbalized reasoning at inference time, but it remains unclear which aspects of task difficulty these extra reasoning tokens address. To investigate this question, we formalize a framework using deterministic finite automata (DFAs). DFAs offer a formalism through which we can characterize task complexity through measurable properties such as run length (number of reasoning steps required) and state-space size (decision complexity). We first show that across different tasks and models of different sizes and training paradigms, there exists an optimal amount of reasoning tokens such that the probability of producing a correct solution is maximized. We then investigate which properties of complexity govern this critical length: we find that task instances with longer corresponding underlying DFA runs (i.e. demand greater latent state-tracking requirements) correlate with longer reasoning lengths, but, surprisingly, that DFA size (i.e. state-space complexity) does not. We then demonstrate an implication of these findings: being able to predict the optimal number of reasoning tokens for new problems and filtering out non-optimal length answers results in consistent accuracy improvements.

==> array_idx_mult.tex <==
\section{Array Index}
A variant of the following is generated every time, with the following parameters:\begin{itemize}
    \item $k$: number of states
    \item $m$: multiplicative factor -- each subsequent node is identified as a multiple of $m$
    \item $N$: length of a run through this automata
\end{itemize}

\begin{center}
\begin{tikzpicture}[scale=0.2]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (19.5,-18) circle (3);
\draw [black] (49.5,-17.2) circle (3);
\draw [black] (35.6,-38.5) circle (3);
\draw [black] (65.8,-54.2) circle (3);
\draw [black] (22.176,-16.647) arc (114.13854:68.91651:31.976);
\fill [black] (46.76,-15.99) -- (46.19,-15.24) -- (45.83,-16.17);
\draw (34.38,-13.32) node [above] {$+9$};
\draw [black] (49.294,-20.191) arc (-7.60986:-58.64564:23.444);
\fill [black] (38.25,-37.11) -- (39.2,-37.12) -- (38.68,-36.26);
\draw (46.31,-31.22) node [right] {$+9$};
\draw [black] (32.916,-37.163) arc (-119.63112:-164.07911:27.296);
\fill [black] (20.16,-20.92) -- (19.9,-21.83) -- (20.86,-21.56);
\draw (24.38,-31.71) node [left] {$+9$};
\draw [black] (21.949,-19.732) arc (52.61344:23.67632:40.659);
\fill [black] (34.5,-35.71) -- (34.63,-34.78) -- (33.72,-35.18);
\draw (29.8,-25.51) node [right] {$-9$};
\draw [black] (46.547,-17.726) arc (-80.84729:-96.09766:90.729);
\fill [black] (22.48,-18.37) -- (23.22,-18.95) -- (23.33,-17.96);
\draw (34.55,-19.38) node [below] {$-9$};
\draw [black] (36.315,-35.587) arc (163.70066:130.04385:34.153);
\fill [black] (47.12,-19.03) -- (46.19,-19.16) -- (46.83,-19.92);
\draw (39.88,-25.19) node [left] {$-9$};
\draw [black] (32.662,-39.094) arc (-83.00741:-343.24809:19.38);
\fill [black] (48.86,-14.27) -- (49.11,-13.36) -- (48.15,-13.65);
\draw (13.46,-7.95) node [left] {$+18$};
\draw [black] (19.917,-15.032) arc (167.60264:-91.31288:19.57);
\fill [black] (38.58,-38.8) -- (39.37,-39.32) -- (39.39,-38.32);
\draw (54.99,-5.73) node [right] {$+18$};
\draw [black] (51.172,-19.687) arc (29.33225:-206.2772:18.778);
\fill [black] (17.96,-20.57) -- (17.16,-21.07) -- (18.06,-21.51);
\draw (35.33,-48.21) node [below] {$+18$};
\draw [black] (38.104,-40.131) arc (84.65581:-203.34419:2.25);
\draw (40.04,-44.81) node [below] {$0$};
\fill [black] (35.83,-41.48) -- (35.26,-42.23) -- (36.25,-42.32);
\draw [black] (51.591,-15.065) arc (163.32351:-124.67649:2.25);
\draw (56.63,-14.21) node [right] {$0$};
\fill [black] (52.47,-17.56) -- (53.09,-18.27) -- (53.38,-17.31);
\draw [black] (51.579,-15.053) arc (163.65382:-124.34618:2.25);
\fill [black] (52.47,-17.54) -- (53.1,-18.25) -- (53.38,-17.29);
\draw [black] (16.996,-16.369) arc (264.65879:-23.34121:2.25);
\draw (15.06,-11.69) node [above] {$0$};
\fill [black] (19.27,-15.02) -- (19.84,-14.27) -- (18.85,-14.18);
\end{tikzpicture}
\end{center}


\begin{verbatim}
You are given a length-3 array and must track the index of a 0-indexed
pointer to the array. The pointer undergoes several modifications. The 
pointer wraps around the length of the array on both ends, so when it 
reaches 3 it becomes 0, when it reaches 4 it becomes 1, when it 
reaches -1 it becomes 2, etc. What is the index of the pointer after 
all the modifications are complete? Provide the answer in the range 
[0, 3).

pointer = 0
pointer += 18
pointer += 0
pointer -= 9
pointer -= 9
\end{verbatim}
In the above example, $k=3$, $m=9$, $N=4$.

We show that LLMs use test-time compute to navigate their internal world model for a task. 


\paragraph{Preliminary: Task performance increases with test-time tokens until a point.}
Across tasks and models, task performance generally improves with the number of test time tokens generated, as seen in Figure~\ref{fig:idx_mult_curves}.

\begin{figure}
    \centering
    \includegraphics[width=.33\textwidth]{images/idx_mult/m15917_k9_N10_gemma-2-9b.png}\hfill
    \includegraphics[width=.33\textwidth]{images/idx_mult/m15917_k5_N16_Ministral-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/idx_mult/m15917_k17_N24_Qwen2.5-32B.png}\hfill
    \caption{Task performance (y-axis) correlates with more test-time tokens (x-axis). The improvement sees diminishing returns after a certain amount of extra test-time tokens.}\label{fig:idx_mult_curves}
\end{figure}


\paragraph{(1) The number of test-time tokens to reach peak performance correlates with the length of the run ($N$) but not parameters of the world model DFA ($k$, $m$).}
We plot the amount of test-time tokens at which peak performance is achieved against parameters of the task in Figure~\ref{fig:idx_mult_diminish}.
(Details: across $(k, m, N)$ experiments, we get the peak tt-toks number. Then for each distinct value of the x-axis factor, we average the peak tt-toks. Per model, we then normalize these averaged values to be in the range [0, 1]. These normalized averaged values are the plotted points. We then measure the mean-squared error against the linear line from [0, 1].)


\begin{figure}
    \centering
    \includegraphics[width=.3\textwidth]{images/idx_mult/T0_diminish_k.png}\hfill
    \includegraphics[width=.33\textwidth]{images/idx_mult/T0_diminish_m.png}\hfill
    \includegraphics[width=.33\textwidth]{images/idx_mult/T0_diminish_N.png}\hfill
    % \\[\smallskipamount]
    \caption{The number of test-time tokens at which peak performance is achieved correlates with number of transitions per task instance ($N$) but not strongly with properties of the DFA itself ($k$, $m$). \textcolor{red}{include slope, we want close to 1}}\label{fig:index_N}
\end{figure}
\textcolor{red}{implication}

\paragraph{(3)  The number of test-time tokens to reach peak performance correlates with $k$ .}
Figure~\ref{fig:index_decay_k} showed that the larger the state space of the underlying world model, the higher the error rate. 
Figure~\ref{fig:index_k} shows that as the size of the true task automata increases, the number of tt-toks to reach peak performance generally increases as well. However, this effect is \textit{only for tasks that require state reasoning}-- it is nonexistent for $N=1$ and more pronounced for larger $N$. \newline
$\rightarrow$ This suggests that more tt-toks can be used to reduce the error rate of transitions, and this reduction is more pronounced in tasks that mandate state-tracking and have more states in its underlying world model.


\begin{figure}
    \centering
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt2_3.1-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt2_gemma-2-9b.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt2_Ministral-8B.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt4_3.1-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt4_gemma-2-9b.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt4_Ministral-8B.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt6_3.1-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt6_gemma-2-9b.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt2_Ministral-8B.png}\hfill
    \caption{Number of tt-tokens to reach peak performance (y-axis) vs. $k$ (x-axis) for a range of models (columns) and transition difficulties ($t$, rows). The increase in peak tt-toks with $k$ is nonexistent for $N=1$ (blue) and is increasingly apparent for larger $N$.}\label{fig:index_k}
\end{figure}

\celine{We need some more robust quantitative measures for the claims made above. Statistical significance tests, percentages, etc...}

\paragraph{(4) Larger models exhibit the same curves at higher performance.}Figure~\ref{fig:index_largesmall} shows that they are only comparable when $N=1$, i.e. there is no state tracking necessary for the task. 
Larger models using few test-time tokens cannot perform as well as their smaller counterparts that do leverage test-time tokens. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/index/byModel_k10_t4_N24_T0.9.png}\hfill
    \includegraphics[width=0.5\linewidth]{images/index/byModel_k30_t2_N24_T0.9.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=0.5\linewidth]{images/index/byModel_k30_t6_N16_T0.9.png}\hfill
    \includegraphics[width=0.5\linewidth]{images/index/byModel_k30_t4_N24_T0.9.png}\hfill
    \caption{All model sizes (Qwen7b yellow; 13b, brown; 13B, blue) exhibit the same patterns as discussed, but large models exhibit the curves at higher performance and later in the performance curve.}
    \label{fig:index_largesmall}
\end{figure}

\paragraph{Some other observations}
\begin{itemize}
    \item Models must be at least above a certain size and instruction-tuned to do well on this task. Also they should be more recent models (e.g. Llama 3.1 8B > Llama 2 13B).
    \item We don't need to explicitly request longer or shorter generations-- high temperatures and sampling enough takes care of that for us. Still, some models tend to produce short generations without CoT. See Figure~\ref{fig:gen_length}
    \item 
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/index/lengthvsrequested_boxplot_T0.9.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> array_index.tex <==
\section{Array Index}
A variant of the following is generated every time, with the following parameters:\begin{itemize}
    \item $k$: number of states
    \item $t$: edges going up to $t//2$ states forward and backward
    \item $N$: length of a run through this automata
\end{itemize}

\begin{center}
\begin{tikzpicture}[scale=0.2]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (14.2,-20.5) circle (3);
\draw (14.2,-20.5) node {$0$};
\draw [black] (14.2,-20.5) circle (2.4);
\draw [black] (28.6,-8.4) circle (3);
\draw (28.6,-8.4) node {$1$};
\draw [black] (48.4,-8.4) circle (3);
\draw (48.4,-8.4) node {$2$};
\draw [black] (60.5,-20.5) circle (3);
\draw (60.5,-20.5) node {$3$};
\draw [black] (48.4,-32.7) circle (3);
\draw (48.4,-32.7) node {$4$};
\draw [black] (29.2,-32.7) circle (3);
\draw (29.2,-32.7) node {$5$};
\draw [black] (27.227,-11.064) arc (-31.38582:-68.535:20.842);
\fill [black] (27.23,-11.06) -- (26.38,-11.49) -- (27.24,-12.01);
\draw (23.85,-16.66) node [below] {$1$};
\draw [black] (13.702,-17.545) arc (-175.15556:-325.87676:18.214);
\fill [black] (46.93,-5.79) -- (46.89,-4.85) -- (46.07,-5.41);
\draw (24.86,1.69) node [above] {$2$};
\draw [black] (31.39,-7.303) arc (107.76597:72.23403:23.301);
\fill [black] (45.61,-7.3) -- (45,-6.58) -- (44.7,-7.54);
\draw (38.5,-5.69) node [above] {$1$};
\draw [black] (51.315,-9.085) arc (70.59114:19.40886:13.915);
\fill [black] (59.81,-17.59) -- (60.02,-16.66) -- (59.08,-17);
\draw (57.55,-11.89) node [above] {$1$};
\draw [black] (49.274,-29.835) arc (157.55038:112.92119:15.649);
\fill [black] (49.27,-29.83) -- (50.04,-29.29) -- (49.12,-28.9);
\draw (52.1,-23.32) node [left] {$1$};
\draw [black] (17.18,-20.8) arc (78.65984:23.09495:15.374);
\fill [black] (17.18,-20.8) -- (17.87,-21.45) -- (18.06,-20.47);
\draw (24.87,-23.45) node [above] {$1$};
\draw [black] (29.911,-5.706) arc (149.01887:-10.56338:17.059);
\fill [black] (61.31,-17.61) -- (61.94,-16.92) -- (60.96,-16.74);
\draw (51.53,1.99) node [above] {$2$};
\draw [black] (51.102,-7.108) arc (109.52976:-109.52976:14.262);
\fill [black] (51.1,-33.99) -- (51.69,-34.73) -- (52.02,-33.79);
\draw (70.63,-20.55) node [right] {$2$};
\draw [black] (45.611,-33.799) arc (-72.33175:-107.66825:22.44);
\fill [black] (31.99,-33.8) -- (32.6,-34.52) -- (32.9,-33.56);
\draw (38.8,-35.36) node [below] {$1$};
\draw [black] (61.479,-23.331) arc (13.97107:-151.38174:16.818);
\fill [black] (30.4,-35.45) -- (30.34,-36.39) -- (31.22,-35.91);
\draw (52.22,-43.58) node [below] {$2$};
\draw [black] (47.039,-35.37) arc (-31.73679:-187.5284:18.175);
\fill [black] (13.56,-23.43) -- (12.96,-24.16) -- (13.95,-24.29);
\draw (24.56,-43.46) node [below] {$2$};
\draw [black] (26.641,-34.256) arc (-64.43979:-292.73136:14.955);
\fill [black] (25.97,-6.97) -- (25.42,-6.2) -- (25.04,-7.12);
\draw (4.7,-21.14) node [left] {$2$};
\draw [black] (11.52,-21.823) arc (-36:-324:2.25);
\draw (6.95,-20.5) node [left] {$0$};
\fill [black] (11.52,-19.18) -- (11.17,-18.3) -- (10.58,-19.11);
\draw [black] (26.877,-5.959) arc (242.95298:-45.04702:2.25);
\draw (27.15,-1.14) node [above] {$0$};
\fill [black] (29.49,-5.55) -- (30.3,-5.06) -- (29.41,-4.61);
\draw [black] (49.016,-5.476) arc (195.84277:-92.15723:2.25);
\draw (53.58,-2.6) node [above] {$0$};
\fill [black] (51.1,-7.11) -- (52,-7.37) -- (51.73,-6.41);
\draw [black] (63.37,-19.669) arc (133.87533:-154.12467:2.25);
\draw (67.87,-21.94) node [right] {$0$};
\fill [black] (62.91,-22.27) -- (63.1,-23.2) -- (63.82,-22.5);
\draw [black] (50.473,-34.853) arc (71.65012:-216.34988:2.25);
\draw (51.31,-39.67) node [below] {$0$};
\fill [black] (47.95,-35.65) -- (47.23,-36.26) -- (48.17,-36.57);
\draw [black] (29.698,-35.647) arc (37.31696:-250.68304:2.25);
\draw (26.43,-39.72) node [below] {$0$};
\fill [black] (27.16,-34.89) -- (26.22,-34.97) -- (26.83,-35.77);
\draw [black] (26.391,-31.65) arc (-113.81595:-144.42926:25.859);
\fill [black] (26.39,-31.65) -- (25.86,-30.87) -- (25.46,-31.78);
\draw (19.18,-28.55) node [below] {$-1$};
\draw [black] (47.634,-35.597) arc (-19.47504:-199.79016:18.408);
\fill [black] (47.63,-35.6) -- (46.9,-36.18) -- (47.84,-36.52);
\draw (22.87,-47.34) node [below] {$-2$};
\draw [black] (62.127,-23.016) arc (27.98617:-165.39685:17.519);
\fill [black] (62.13,-23.02) -- (62.06,-23.96) -- (62.94,-23.49);
\draw (54.28,-48.09) node [below] {$-2$};
\draw [black] (31.837,-31.278) arc (113.42282:66.57718:17.515);
\fill [black] (45.76,-31.28) -- (45.23,-30.5) -- (44.83,-31.42);
\draw (38.8,-29.33) node [above] {$-1$};
\draw [black] (59.872,-23.427) arc (-18.38835:-71.14009:13.665);
\fill [black] (59.87,-23.43) -- (59.15,-24.03) -- (60.09,-24.34);
\draw (57.13,-30.22) node [right] {$-1$};
\draw [black] (50.858,-6.688) arc (119.46144:-119.46144:15.921);
\fill [black] (50.86,-6.69) -- (51.8,-6.73) -- (51.31,-5.86);
\draw (75.11,-20.55) node [right] {$-2$};
\draw [black] (57.771,-19.26) arc (-118.6523:-151.3477:20.427);
\fill [black] (49.64,-11.13) -- (49.59,-12.07) -- (50.46,-11.59);
\draw (51.77,-16.25) node [below] {$-1$};
\draw [black] (45.498,-9.156) arc (-77.96636:-102.03364:33.565);
\fill [black] (31.5,-9.16) -- (32.18,-9.81) -- (32.39,-8.83);
\draw (38.5,-10.39) node [below] {$-1$};
\draw [black] (15.972,-18.08) arc (141.21829:118.86089:33.483);
\fill [black] (15.97,-18.08) -- (16.86,-17.77) -- (16.08,-17.14);
\draw (19.19,-12.93) node [above] {$-1$};
\draw [black] (29.119,-5.449) arc (165.18025:-26.72476:17.716);
\fill [black] (29.12,-5.45) -- (29.81,-4.8) -- (28.84,-4.55);
\draw (53.78,7.11) node [above] {$-1$};
\draw [black] (12.72,-17.894) arc (-154.9782:-346.05412:18.753);
\fill [black] (12.72,-17.89) -- (12.83,-16.96) -- (11.93,-17.38);
\draw (22.24,8.26) node [above] {$-2$};
\draw [black] (26.903,-34.623) arc (-55.17835:-301.9928:16.795);
\fill [black] (26.9,-34.62) -- (25.96,-34.67) -- (26.53,-35.49);
\draw (-0.01,-21.26) node [left] {$-2$};
\end{tikzpicture}
\end{center}


\begin{verbatim}
You are given a length-6 array and must track the index of a 0-indexed
pointer to the array. The pointer undergoes several modifications. The 
pointer wraps around the length of the array on both ends, so when it 
reaches 6 it becomes 0, when it reaches 7 it becomes 1, when it 
reaches -1 it becomes 5, etc. What is the index of the pointer after 
all the modifications are complete? Provide the answer in the range 
[0, 6).

pointer = 0
pointer += 2
pointer += 0
pointer -= 1
pointer -= 1
\end{verbatim}
In the above example, $k=6$, $t=4$, $N=4$.

% To show that there is a correlation between test-time compute and performance with respect to the complexity of the underlying task DFA, w
We show that LLMs build and use an internal world model that resembles a probabilistic semiautomaton consistent with the true underlying task automaton. We further 
\textbf{show that the complexity of the underlying task automaton is reflected in the LLM's task performance relative to the number of test-time tokens used.}


\paragraph{(0) Task performance follows that of a probabilistic semiautomaton.} 
% How do we know the LLM world model resembles the DFA? 
% To perform the task according to the described DFA would be to execute the ground truth run that produced the task instance. 
% One sign that the LLM builds and traverses an internal world model consistent with the DFA is if for a given-complexity DFA (same states and transitions), task completion accuracy follows an exponential decay according to the length of the ground truth run. 
For a given underlying automaton and model, LLM task performance degrades as a function of $N$. Specifically, this degradation approximately follows an exponential decay consistent with that of a probabilistic semiautomaton as defined in Equation~\ref{eqn:exp_decay}.
The error rate $d$ tends to be higher for automata with more states ($k$), as seen in Figure~\ref{fig:index_decay_k}. \newline
$\rightarrow$ This implies that \textbf{LLMs generally infer a probabilistic semiautomaton consistent with the underlying true world model automaton, and that automata with more states (more complex world models) result in a higher error rate.}

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{images/index/correctness_k_t2_gemma-2-9b_T0.9.png}\hfill
    \includegraphics[width=.5\textwidth]{images/index/correctness_k_t4_3.1-8B_T0.9.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=.5\textwidth]{images/index/correctness_k_t4_Ministral-8B_T0.9.png}\hfill
    \includegraphics[width=.5\textwidth]{images/index/correctness_k_t6_Qwen2.5-7B_T0.9.png}\hfill
    \caption{As the instance complexity $N$ increases (x axis), performance (y axis) drops following an exponential decay according to the model and DFA state space size ($k$, line darkness). Fitted exponential decay curves are overlaid in dashed black lines.}\label{fig:index_decay_k}
\end{figure}


\paragraph{(1) Task performance increases with test-time tokens up until a point.}
Across models, $k$, $t$, and $N$, task performance improves with the number of test time tokens generated. Beyond some number of test-time tokens, performance can begin to decrease, as seen in Figure~\ref{fig:index_curves}.
In the context of automata as world models, this resembles a run that has gone awry with more test-time tokens. This could happen by transitioning to an incorrect state or inferring an incorrect world model to start with.

\begin{figure}
    \centering
    \includegraphics[width=.33\textwidth]{images/index/byModel_k5_t2_N1_T0.9.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/byModel_k5_t2_N10_T0.9.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/byModel_k5_t4_N10_T0.9.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=.33\textwidth]{images/index/byModel_k10_t2_N10_T0.9.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/byModel_k10_t6_N16_T0.9.png}\hfill
    % \includegraphics[width=.33\textwidth]{images/index/byModel_k30_t2_N10_T0.9.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/byModel_k30_t6_N24_T0.9.png}\hfill
    \caption{Task accuracy (y-axis) improves with more test-time tokens (x-axis) up until a point, at which more test-time tokens can reduce performance. This is consistent with previous literature finding that on some tasks, humans and LLMs both suffer from additional verbal reasoning~\cite{liu2024mindstepbystep}.}\label{fig:index_curves}
\end{figure}



\paragraph{(2) The number of test-time tokens to reach peak performance correlates with $N$.}
Figure~\ref{fig:index_N} shows that across different DFAs and models, as the complexity of the task instance increases ($N$ is the length of the correct DFA run), the number of test-time tokens (tt-toks) to reach peak performance increases. \newline
$\rightarrow$ This suggests that when the task mandates tracking states, each transition uses some amount of compute, and as more transitions are necessary for the task instance, more additional compute is useful for state tracking and inference.

\begin{figure}
    \centering
    \includegraphics[width=.3\textwidth]{images/index/N1101624_k5_t2_3.1-8B_T0.9.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/N1101624_k10_t4_Ministral-8B_T0.9.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/N1101624_k30_t6_gemma-2-9b_T0.9.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=.33\textwidth]{images/index/diminish_N1101624_holdk5_3.1-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_N1101624_holdk10_Ministral-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_N1101624_holdk30_gemma-2-9b.png}\hfill
    \caption{Top: As the number of transitions per task instance ($N$) increases (darker hues), more tokens (x-axis) are necessary to achieve peak performance (y-axis). Bottom: Number of tt-tokens to reach peak performance (y-axis) vs. $N$ (x-axis).}\label{fig:index_N}
\end{figure}


\paragraph{(3)  The number of test-time tokens to reach peak performance correlates with $k$ .}
Figure~\ref{fig:index_decay_k} showed that the larger the state space of the underlying world model, the higher the error rate. 
Figure~\ref{fig:index_k} shows that as the size of the true task automata increases, the number of tt-toks to reach peak performance generally increases as well. However, this effect is \textit{only for tasks that require state reasoning}-- it is nonexistent for $N=1$ and more pronounced for larger $N$. \newline
$\rightarrow$ This suggests that more tt-toks can be used to reduce the error rate of transitions, and this reduction is more pronounced in tasks that mandate state-tracking and have more states in its underlying world model.


\begin{figure}
    \centering
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt2_3.1-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt2_gemma-2-9b.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt2_Ministral-8B.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt4_3.1-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt4_gemma-2-9b.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt4_Ministral-8B.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt6_3.1-8B.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt6_gemma-2-9b.png}\hfill
    \includegraphics[width=.33\textwidth]{images/index/diminish_k51030_holdt2_Ministral-8B.png}\hfill
    \caption{Number of tt-tokens to reach peak performance (y-axis) vs. $k$ (x-axis) for a range of models (columns) and transition difficulties ($t$, rows). The increase in peak tt-toks with $k$ is nonexistent for $N=1$ (blue) and is increasingly apparent for larger $N$.}\label{fig:index_k}
\end{figure}

\celine{We need some more robust quantitative measures for the claims made above. Statistical significance tests, percentages, etc...}

\paragraph{(4) Larger models exhibit the same curves at higher performance.}Figure~\ref{fig:index_largesmall} shows that they are only comparable when $N=1$, i.e. there is no state tracking necessary for the task. 
Larger models using few test-time tokens cannot perform as well as their smaller counterparts that do leverage test-time tokens. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/index/byModel_k10_t4_N24_T0.9.png}\hfill
    \includegraphics[width=0.5\linewidth]{images/index/byModel_k30_t2_N24_T0.9.png}\hfill
    \\[\smallskipamount]
    \includegraphics[width=0.5\linewidth]{images/index/byModel_k30_t6_N16_T0.9.png}\hfill
    \includegraphics[width=0.5\linewidth]{images/index/byModel_k30_t4_N24_T0.9.png}\hfill
    \caption{All model sizes (Qwen7b yellow; 13b, brown; 13B, blue) exhibit the same patterns as discussed, but large models exhibit the curves at higher performance and later in the performance curve.}
    \label{fig:index_largesmall}
\end{figure}

\paragraph{Some other observations}
\begin{itemize}
    \item Models must be at least above a certain size and instruction-tuned to do well on this task. Also they should be more recent models (e.g. Llama 3.1 8B > Llama 2 13B).
    \item We don't need to explicitly request longer or shorter generations-- high temperatures and sampling enough takes care of that for us. Still, some models tend to produce short generations without CoT. See Figure~\ref{fig:gen_length}
    \item 
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/index/lengthvsrequested_boxplot_T0.9.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

